Diversity-based core-set selection for text-to-speech with linguistic and acoustic features

This paper proposes a method for extracting a lightweight subset from a text-to-speech (TTS) corpus ensuring synthetic speech quality. In recent years, methods have been proposed for constructing large-scale TTS corpora by collecting diverse data from massive sources such as audiobooks and YouTube. Although these methods have gained significant attention for enhancing the expressive capabilities of TTS systems, they often prioritize collecting vast amounts of data without considering practical constraints like storage capacity and computation time in training, which limits the available data quantity. Consequently, the need arises to efficiently collect data within these volume constraints. To address this, we propose a method for selecting the core subset~(known as \textit{core-set}) from a TTS corpus on the basis of a \textit{diversity metric}, which measures the degree to which a subset encompasses a wide range. Experimental results demonstrate that our proposed method performs significantly better than the baseline phoneme-balanced data selection across language and corpus size.

==> fig/actual_mos.tex <==

\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{image/actual_mos.pdf}
\vspace{-7mm}
\caption{Cumulative histogram of speaker-wise MOS for models trained on the JVS corpus.}
\label{fig:subjective_columtive_histogram}
\vspace{-5mm}
\end{figure}


==> fig/diversity_compare.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{image/diversity_compare.pdf}
\vspace{-7mm}
\caption{Comparison of cumulative histograms of speaker-wise pseudo-MOS for each feature.}
\label{fig:diversity_columtive_histogram}
\vspace{-3mm}
\end{figure}

==> fig/foreign_histogram.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{image/foreign_mos.pdf}
\vspace{-7mm}
\caption{Cumulative histogram of speaker-wise MOS for models trained on the AISHELL-3 corpus and the LibriTTS-R corpus.}
\label{fig:subjective_columtive_histogram}
\vspace{-3mm}
\end{figure}

==> fig/joint_pseudo-MOS.tex <==
\begin{figure}[t]
  \centering
  \begin{minipage}{1\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{image/pseudo_mos.pdf}
    \vspace{-5mm}
    \subcaption{Comparison between the balance methods and our method.}
    \label{fig:all_columtive_histogram}
  \end{minipage}
  \vfill
  \begin{minipage}{1\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{image/diversity_compare.pdf}
    \vspace{-5mm}
    \subcaption{Ablation study about features.}
    \label{fig:diversity_columtive_histogram}
  \end{minipage}
  \vspace{-3mm}
  \caption{Cumulative histogram of speaker-wise pseudo-MOS for each model. The values on the $y$-axis represent the number of speakers with pseudo-MOS scores higher than the values on the $x$-axis.}
  \vspace{-4.5mm}
\end{figure}


==> temp_takamichi.tex <==
\newpage
\section{takamichi's memo (ato de kesu)}
    \textbf{Multi-speaker and noise-robust TTS.}
        Multi-speaker TTS uses speaker representations to control the speaker of the synthetic speech~\cite{DeepVoice2,DeepVoice3}. The $x$-vector used in automatic speaker verification (ASV) is an efficient approach for the control; we follow this in this paper. Also, a few-shot speaker adaptation, voice building of a new speaker from a small amount of speech data~\cite{cooperZeroShotMultiSpeakerEmbedding}, is the promising application of multi-speaker TTS. To increase the number of speakers using diverse training data, there exists some noise-aware TTS training~\cite{DenoiSpeech,DRSpeech,DenoiSpeech的なやつ}.
    
    \textbf{Building TTS corpus on ASR corpus.}
        The use of more speakers' data in training increases the speaker variation in TTS. Methods based on data refinement and selection of ASR corpora have been proposed for this purpose. The well-known examples are based on acoustic noise~\cite{話者認証からMultiSpeakerへの転移} and text label noise (i.e., a mismatch between text and speech)~\cite{LibriTTS}. These methodologies help construct a TTS corpus from an ASR corpus. However, these processes are based only on data quality and are performed independently of the TTS model. These methodologies are not appropriate considering the noise robustness of the TTS model, which we desribed above.
    
        Related to above, dark data has the potential to build massive speech corpora almost fully automatically, and indeed, successful examples of this have been reported in the construction of ASR corpora~\cite{galvez2021peoplespeech,chen2021gigaspeech}. In this paper, we focus on only the speaker variation but expect that it can be extended to other speech-related factors, e.g., style.
    
    \textbf{Prediction of perceptual quality in synthetic speech.}
        Methods for automatically predicting the subjective evaluation score from synthetic speech have been studied to reduce the evaluation cost for TTS~\cite{moller10mosprediction,patton16automos}. The challenge in automatic prediction is generalization performance, i.e., the robustness of the prediction against divergence between the training and evaluation data. The recent deep learning-based models (used in this paper) have relatively good accuracy in predicting the relative rank between speech samples, although the accuracy of predicting the value itself was reduced~\cite{huang22voicemos}.
        
